Nonlinear Predictive Control on a Heterogeneous Computing Platform

We propose an implementation of an interior-point-based nonlinear predictive controller on a heterogeneous processor. The workload can be split between a general-purpose CPU and a field-programmable gate array to trade off the contradicting design objectives of control performance and computational resource usage. A new way of exploiting the structure of the KKT matrix yields significant memory savings. We report an 18x memory saving, compared to existing approaches, and a 36x speedup over a software implementation with an ARM Cortex-A9 processor. We also introduce a new release of Protoip, which abstracts low-level details of heterogeneous programming and allows processor-in-the-loop verification.

==> resource_performance.tex <==
% !TEX root = ../root.tex
\section{Synthesis and simulation results}

Four implementations (software only and three heterogeneous) of Algorithm~\ref{alg:ip} were deployed and tested with Protoip. Single precision floating point data arithmetic was used, clocking the CPU and FPGA  at 667\,MHz and 100\,MHz, respectively. The benchmark plant model and OCP parameters are given in Appendix~\ref{sec:crane_ode}. For the considered example, the pure software implementations were not able to compute optimal solution within one sampling instant  $T_s=150$\,ms and $n_{iter} = 15$, as can be seen in Table~\ref{tab:time_comparison}. Speeding up certain parts of the computational workload on the FPGA and allocating two MAC units for matrix-vector multiplication resulted in a reduced computational time and hence implementing  the algorithm online. 
\begin{table}[tb]
\caption{Algorithm execution times with heterogeneous implementations. Feasible designs are highlighted with a gray background.}
\centering
\begin{tabular}{>{\centering\arraybackslash} p{0.02\textwidth} | p{0.02\textwidth} | p{0.03\textwidth} | p{0.02\textwidth} | p{0.03\textwidth} | p{0.02\textwidth} | p{0.03\textwidth} | p{0.02\textwidth}}
\toprule
N & \multicolumn{1}{c|}{Software, ms} & \multicolumn{2}{p{0.08\textwidth}|}{Mat-vec multiplication on FPGA, ms} & \multicolumn{2}{p{0.08\textwidth}}{Lanczos kernel on FPGA, ms} & \multicolumn{2}{|p{0.08\textwidth}}{Linear solver on FPGA, ms} \\ \hline
2 & \multicolumn{1}{c|}{416} & \multicolumn{2}{c|}{\cellcolor{gray} 144}&  \multicolumn{2}{c|}{\cellcolor{gray} 78} & \multicolumn{2}{c|}{\cellcolor{gray} 48} \\ 
3 & \multicolumn{1}{c|}{600} & \multicolumn{2}{c|}{227}&  \multicolumn{2}{c|}{\cellcolor{gray} 125} &   \multicolumn{2}{c|}{\cellcolor{gray} 68} \\ 
4 & \multicolumn{1}{c|}{1043} & \multicolumn{2}{c|}{373}&  \multicolumn{2}{c|}{195}& \multicolumn{2}{c|}{\cellcolor{gray} 109} \\ 
5 & \multicolumn{1}{c|}{1316} & \multicolumn{2}{c|}{502}&  \multicolumn{2}{c|}{265}&  \multicolumn{2}{c|}{\cellcolor{gray}  135} \\ 
6 & \multicolumn{1}{c|}{2033} & \multicolumn{2}{c|}{695}& \multicolumn{2}{c|}{366} & \multicolumn{2}{c|}{191} \\
\bottomrule
\end{tabular}
\label{tab:time_comparison}
\end{table}

The trade-off between the closed-loop  performance and processor resource usage for the feasible designs from Table~\ref{tab:time_comparison} is illustrated in Figure~\ref{fig:heterogeneous_tradeoffs}. 
\begin{figure}[tb]
        \centering
        \includegraphics[width=\columnwidth]{figures/performance_resource/performacne_vs_resource_usage.eps} 
        \caption{Trading off closed-loop performance against resource usage by splitting the workload between software and hardware.}
        \label{fig:heterogeneous_tradeoffs}
\end{figure}
We measure closed-loop performance based on a PIL simulation with the cost function
\begin{equation}
	 V(\textrm{$\mbox{u}$,$\mbox{x}$}) = \sum_{k=0}^{N_{sim}-1}(\frac{1}{2}\mbox{x}_{k}^{T} Q_{d}\mbox{x}_{k} + \frac{1}			{2}\mbox{u}_{k}^{T} R_{d}\mbox{u}_{k} + \mbox{x}_{k}^{T} S_{d}\mbox{u}_{k}),
	\label{cl_cost}
\end{equation}
where $\textrm{u}_{k}$ is an input to the plant and $\textrm{x}_{k}$ is a state of the plant at sampling instance $k$. The number of simulation samples $N_{sim}$ is chosen to reflect convergence or divergence of the controlled plant. Resource usage is measured as geometric mean of relative utilization of each resource type, namely LUT, FF, block RAM and DSP. Three out of seven considered designs are Pareto-optimal. The notable point  is that Pareto-optimal designs  are achieved by splitting the workload between software and hardware in different ways, which justifies the flexibility of the software-hardware splitting of the proposed implementation.

%For all heterogeneous implementations FPGA clock frequency was set to 100\,MHz. We present the maximum possible frequencies  reported by the synthesis tool for reference only (Table~\ref{tab:time_comparison}). Note that for all considered designs, the highest possible frequency is above  500\,MHz, which is higher compared to existing implementations of predictive controllers on reconfigurable platforms~\citep{juan_fpga_qp}. This is due to the fact that, with the proposed implementation, sequential part of the algorithm, that often limits FPGA clock frequency is implemented on CPU.

%\begin{table*}[tb]
%\centering
%\caption{Algorithm execution times with heterogeneous implementations. For all considered implementations CPU clock rate is 667\,MHz and FPGA clock frequency is 100\,MHz. Two MAC units were allocated for matrix-vector multiplication. $T_s=150$\,ms, $n_{iter} = 15$, feasible designs are highlighted with a gray background.}
%\begin{tabular}{>{\centering\arraybackslash} p{0.02\textwidth} | p{0.05\textwidth} | p{0.03\textwidth} | p{0.17\textwidth} | p{0.03\textwidth} | p{0.15\textwidth} | p{0.03\textwidth} | p{0.15\textwidth}}
%\toprule
%N & \multicolumn{1}{c|}{Software} & \multicolumn{2}{p{0.20\textwidth}|}{Heterogeneous 1 (Mat-vec multiplication on FPGA)} & \multicolumn{2}{p{0.18\textwidth}}{Heterogeneous 2 (Lanczos kernel on FPGA)} & \multicolumn{2}{|p{0.18\textwidth}}{Heterogeneous 3 (Linear solver on FPGA)} \\ \hline
%{} & \multicolumn{1}{c|}{time, ms} & \multicolumn{1}{c|}{time, ms} & \multicolumn{1}{p{0.15\textwidth}|}{Max FPGA clock rate, MHz} & \multicolumn{1}{c|}{time, ms} & \multicolumn{1}{p{0.15\textwidth}|}{Max FPGA clock rate, MHz} & \multicolumn{1}{c|}{time, ms} & \multicolumn{1}{p{0.15\textwidth}|}{Max FPGA clock rate, MHz} \\ \hline
%2 & \multicolumn{1}{c|}{416} & \multicolumn{1}{c|}{\cellcolor{gray} 144}& \multicolumn{1}{c|}{\cellcolor{gray} 1414} &  \multicolumn{1}{c|}{\cellcolor{gray} 78}  &  \multicolumn{1}{c|}{\cellcolor{gray} 639} & \multicolumn{1}{c|}{\cellcolor{gray} 48} &  \multicolumn{1}{c}{\cellcolor{gray} 881}\\ 
%3 & \multicolumn{1}{c|}{600} & \multicolumn{1}{c|}{227}& \multicolumn{1}{c|}{1414} &  \multicolumn{1}{c|}{\cellcolor{gray} 125} &  \multicolumn{1}{c|}{\cellcolor{gray} 639} & \multicolumn{1}{c|}{\cellcolor{gray} 68} &   \multicolumn{1}{c}{\cellcolor{gray} 1582} \\ 
%4 & \multicolumn{1}{c|}{1043} & \multicolumn{1}{c|}{373}& \multicolumn{1}{c|}{639}& \multicolumn{1}{c|}{195}& \multicolumn{1}{c|}{1011}&\multicolumn{1}{c|}{\cellcolor{gray} 109}&  \multicolumn{1}{c}{\cellcolor{gray} 737}\\ 
%5 & \multicolumn{1}{c|}{1316} & \multicolumn{1}{c|}{502}& \multicolumn{1}{c|}{639}& \multicolumn{1}{c|}{265}& \multicolumn{1}{c|}{1011}& \multicolumn{1}{c|}{\cellcolor{gray}  135}&  \multicolumn{1}{c}{\cellcolor{gray} 923}\\ 
%6 & \multicolumn{1}{c|}{2033} & \multicolumn{1}{c|}{695}& \multicolumn{1}{c|}{1089}& \multicolumn{1}{c|}{366}&\multicolumn{1}{c|}{729}& \multicolumn{1}{c|}{191}& \multicolumn{1}{c}{1202}\\
%\bottomrule
%\end{tabular}
%\label{tab:time_comparison}
%\end{table*}


